Certified dimension reduction in nonlinear Bayesian inverse problems

We propose a dimension reduction technique for Bayesian inverse problems with nonlinear forward operators, non-Gaussian priors, and non-Gaussian observation noise. The likelihood function is approximated by a ridge function, i.e., a map which depends non-trivially only on a few linear combinations of the parameters. We build this ridge approximation by minimizing an upper bound on the Kullback--Leibler divergence between the posterior distribution and its approximation. This bound, obtained via logarithmic Sobolev inequalities, allows one to certify the error of the posterior approximation. Computing the bound requires computing the second moment matrix of the gradient of the log-likelihood function. In practice, a sample-based approximation of the upper bound is then required. We provide an analysis that enables control of the posterior approximation error due to this sampling. Numerical and theoretical comparisons with existing methods illustrate the benefits of the proposed methodology.

==> biblio.tex <==
\begin{thebibliography}{10}

\bibitem{Agapiou2017}
  {\sc S.~Agapiou, O.~Papaspiliopoulos, D.~Sanz-Alonso, and A.~Stuart},
{\em {Importance sampling: intrinsic dimension and computational cost}}, 
Statistical Science, 32 (2017), pp.~405--431.

\bibitem{bakry1985diffusions}
{\sc D.~Bakry, M.~{\'{E}}mery, and M.~I.~{\'{E}}. Mery}, {\em {Diffusions
  hypercontractives}}, in S{\{}{\'{e}}{\}}minaire de Probabilit{\{}{\'{e}}{\}}s
  XIX 1983/84, vol.~19, Springer, 1985, pp.~177--206.

\bibitem{Banerjee2005}
{\sc A.~Banerjee, X.~Guo, and H.~Wang}, {\em {On the optimality of conditional
  expectation as a Bregman predictor}}, IEEE Transactions on Information
  Theory, 51 (2005), pp.~2664--2669.

\bibitem{beskos2017multilevel}
{\sc A.~Beskos, A.~Jasra, K.~Law, Y.~Marzouk and Y.~Zhou}, {\em {Multilevel sequential Monte Carlo with 
  dimension-independent likelihood-informed proposals}}, SIAM/ASA Journal on Uncertainty Quantification, 6 (2018), pp.~762--786.
 
\bibitem{Blanchard2007}
{\sc G.~Blanchard, O.~Bousquet, and L.~Zwald}, {\em {Statistical properties of
  kernel principal component analysis}}, Machine Learning, 66 (2007),
  pp.~259--294.

\bibitem{bobkov2000brunn}
{\sc S.~G. Bobkov and M.~Ledoux}, {\em {From Brunn-Minkowski to Brascamp-Lieb
  and to logarithmic sobolev inequalities}}, Geometric {\&} Functional Analysis
  GAFA, 10 (2000), pp.~1028--1052.

\bibitem{boucheron2013concentration}
{\sc S.~Boucheron, G.~Lugosi, and P.~Massart}, {\em {Concentration
  inequalities: A nonasymptotic theory of independence}}, Oxford university
  press, 2013.
  
\bibitem{Cohen2012b}
{\sc A.~Cohen, I.~Daubechies, R.~DeVore, G.~Kerkyacharian, and D.~Picard}, {\em
  {Capturing Ridge Functions in High Dimensions from Point Queries}},
  Constructive Approximation, 35 (2012), pp.~225--243.

\bibitem{Conrad2016}
{\sc P.~Conrad, Y.~Marzouk, N.~Pillai, and A.~Smith},
{\em {Accelerating asymptotically exact MCMC for computationally
    intensive models via local approximations}},
Journal of the American Statistical Association, 111 (2016), pp.~1591–1607.

\bibitem{Constantine2014a}
{\sc P.~G. Constantine, E.~Dow, and Q.~Wang}, {\em {Active subspace methods in
  theory and practice: applications to Kriging surfaces}}, SIAM Journal on
  Scientific Computing, 36 (2014), pp.~A1500--A1524.

\bibitem{Constantine2015}
{\sc P.~G. Constantine, C.~Kent, and T.~Bui-Thanh}, {\em {Accelerating Markov
  chain Monte Carlo with active subspaces}}, SIAM Journal on Scientific
  Computing, 38 (2016), pp.~A2779--A2805.

\bibitem{Cui2014_LIS}
{\sc T.~Cui, J.~Martin, Y.~M. Marzouk, A.~Solonen, and A.~Spantini}, {\em
  {Likelihood-informed dimension reduction for nonlinear inverse problems}},
  Inverse Problems, 29 (2014), pp.~114015.

\bibitem{Cui2015}
{\sc T.~Cui, Y.~Marzouk, and K.~Willcox},
{\em {Data-driven model reduction for the Bayesian solution of inverse problems}},
International Journal for Numerical Methods in Engineering, 102 (2015), pp.~966--990.

\bibitem{Cui2016_DILI}
{\sc T.~Cui, K.~Law, and Y.~M. Marzouk}, {\em Dimension-independent likelihood-informed MCMC},
  Journal of Computational Physics, 304 (2016), pp.~109--137.

\bibitem{Cui2016_joint}
{\sc T.~Cui, Y.~M. Marzouk, K.~Willcox}, {\em
  Scalable posterior approximations for large-scale Bayesian inverse problems via
  likelihood-informed parameter and state reduction}, Journal of Computational 
  Physics, 315 (2016), pp.~363--387.

  
\bibitem{flath2011fast}
{\sc H.~P.~Flath, L.~C.~Wilcox, V.~Ak{\c{c}}elik, J.~Hill, B.~van Bloemen Waanders and O.~Ghattas}, {\em
  Fast algorithms for Bayesian uncertainty quantification in large-scale linear inverse problems based on low-rank partial Hessian approximations}, Journal of Computational 
  SIAM Journal on Scientific Computing, 33 (2011), pp.~407--432.


\bibitem{fornasier2012learning}
{\sc M.~Fornasier, K.~Schnass, and J.~Vybiral}, {\em {Learning functions of few
  arbitrary linear parameters in high dimensions}}, Foundations of
  Computational Mathematics, 12 (2012), pp.~229--262.

\bibitem{Gozlan2013}
{\sc N.~Gozlan, C.~Roberto, and P.~M. Samson}, {\em {Characterization of
  Talagrand's transport-entropy inequalities in metric spaces}}, Annals of
  Probability, 41 (2013), pp.~3112--3139.

\bibitem{gross1975logarithmic}
{\sc L.~Gross}, {\em {Logarithmic sobolev 
 inequalities}}, American Journal of Mathematics, 97 (1975), pp.~1061--1083.

\bibitem{guionnet2003lectures}
{\sc A.~Guionnet and B.~Zegarlinksi}, {\em {Lectures on logarithmic Sobolev
  inequalities}}, S{\'e}minaire de probabilit{\'e}s XXXVI (2003), pp.~1--134.

\bibitem{Haario_etal_2004}
H.~Haario, M.~Laine, M.~Lehtinen, E.~Saksman, and J.~Tamminen.
\newblock {\em {M}arkov chain {M}onte {C}arlo methods for high dimensional inversion
  in remote sensing.}
\newblock {Journal of the Royal Statistical Society: Series B (Statistical
  Methodology)}, 66 (2004), pp.~591--608.

\bibitem{holley1987logarithmic}
{\sc R.~Holley and D.~Stroock}, {\em {Logarithmic Sobolev inequalities and
  stochastic Ising models}}, Journal of Statistical Physics, 46 (1987),
  pp.~1159--1194.

\bibitem{jung1901ueber}
{\sc Jung, Heinrich}, {\em {Ueber die kleinste Kugel, die eine r{\"a}umliche Figur 
  einschliesst.}}, Journal f{\"u}r die reine und angewandte Mathematik, 123 (1901), 
  pp,~241--257.
  
\bibitem{KaipioSomersalo}
{\sc J.~Kaipio and E.~Somersalo},
{\em {Statistical and Computational Inverse Problems}},
Springer (2005).

\bibitem{lamminpaa2017likelihood}
{\sc O.~Lamminp{\"a}{\"a}, M.~Laine, S.~Tukiainen and J.~Tamminen}, {\em {Likelihood 
  informed dimension reduction for inverse problems in remote sensing of atmospheric 
  constituent profiles}}, arXiv preprint (2017) arXiv:1709.02611.
  
\bibitem{ledoux1999concentration}
{\sc M.~Ledoux}, {\em {Concentration of measure and logarithmic Sobolev 
  inequalities}}, S\'eminaire de probabilit\'es XXXIII (1999), pp.~120--216.

\bibitem{Li2015}
{\sc J.~Li}, {\em {A note on the Karhunen-Lo{\`{e}}ve expansions for
  infinite-dimensional Bayesian inverse problems}}, Statistics and Probability
  Letters, 106 (2015), pp.~1--4.

\bibitem{Li2006}
{\sc W.~Li and O.~A. Cirpka}, {\em {Efficient geostatistical inverse methods
  for structured and unstructured grids}}, Water Resources Research, 42 (2006),
  pp.~1--15.
  
  
\bibitem{lieberman2010parameter}
{\sc C.~Lieberman, K.~Willcox and O.~Ghattas}, {\em {Parameter and state model reduction
  for large-scale statistical inverse problems}}, SIAM Journal on Scientific Computing,
  32 (2010), pp.~2523--2542.
  
  
\bibitem{MRF:LRL_2011}
{\sc F.~Lindgren, H.~Rue, and J.~Lindstr\"{o}m},
\newblock {\em An explicit link between {G}aussian fields and
  {G}aussian {M}arkov random fields: the stochastic partial differential
  equation approach.},
\newblock Journal of the Royal Statistical Society: Series B
  (Statistical Methodology), 73 (2011), pp.~423--498.

\bibitem{manzoni2016accurate}
{\sc A.~Manzoni, S.~Pagani and T.~Lassila}, {\em {Accurate solution of Bayesian 
  inverse uncertainty quantification problems combining reduced basis methods
  and reduction error models}}, SIAM/ASA Journal on Uncertainty Quantification, 4 (2016), pp.~380--412.
  
\bibitem{marzouk2009dimensionality}
{\sc Y.~M. Marzouk and H.~N. Najm}, {\em {Dimensionality reduction and
  polynomial chaos acceleration of Bayesian inference in inverse problems}},
  Journal of Computational Physics, 228 (2009), pp.~1862--1902.

\bibitem{Mikosch1998}
{\sc T.~Mikosch and O.~Kallenberg}, {\em {Foundations of Modern Probability}},
  Journal of the American Statistical Association, 93 (1998), p.~1243.

\bibitem{Otto1999}
{\sc F.~Otto and C.~Villani}, {\em {Generalization of an Inequality By
  Talagrand, and Links With the Logarithmic Sobolev Inequality}}, J. of
  Functional Analysis, 173 (1999), pp.~361--400.

\bibitem{OwenBook}
{\sc A.~Owen}, {\em {Monte Carlo theory, methods and examples}},
  2013.
  
% \bibitem{parente2020generalized}
% {\sc Parente, Mario Teixeira and Wallin, Jonas and Wohlmuth, Barbara and others},
%   {\em {Generalized bounds for active subspaces}}, Electronic Journal of Statistics,
%   14 (2020), pp.~917--943.
  
  
\bibitem{pinkus_2015}
{\sc A.~Pinkus}, {\em {Ridge Functions}}, Cambridge Tracts in Mathematics,
  Cambridge University Press, 2015.

\bibitem{Reiss2016}
{\sc M.~Rei{\ss} and M.~Wahl}, {\em {Non-asymptotic upper bounds for the
  reconstruction error of PCA}},  (2016), pp.~1--43.

\bibitem{RobertCasella}
{\sc Robert, C. P. and Casella, G.}, Monte {C}arlo statistical methods. Springer, NYC. 1999.

\bibitem{Russi2010}
{\sc T.~Russi}, {\em {Uncertainty Quantification with Experimental Data and 
  Complex System Models}}, PhD thesis, UC Berkeley, 2010.

\bibitem{rubio2018fast}
{\sc P.~B.~Rubio, F.~Louf and L.~Chamoin}, {\em {Fast model updating coupling
  Bayesian inference and PGD model reduction}}, Computational Mechanics (2018) pp.~1--25  
  
\bibitem{russi2010uncertainty}
{\sc T.~M. Russi}, {\em {Uncertainty quantification with experimental data and
  complex system models}}, PhD thesis, 2010.

\bibitem{Spantani2015}
{\sc A.~Spantini, A.~Solonen, T.~Cui, J.~Martin, L.~Tenorio, and Y.~Marzouk},
  {\em {Optimal Low-rank Approximations of Bayesian Linear Inverse Problems}},
  SIAM Journal on Scientific Computing, 37 (2015), pp.~A2451--A2487.

\bibitem{Stuart2010}
{\sc A.~Stuart},
{\em {Inverse problems: A Bayesian perspective}},
Acta Numerica, 19 (2010), pp.~451--559.

\bibitem{Tamminen_2004}
{\sc J.~Tamminen}, 
\newblock {\em Adaptive Markov chain Monte Carlo algorithms with geophysical applications}, 
Ph.D. thesis, Finnish Meteorologocal Institute, 2004.

\bibitem{teh2007collapsed}
{\sc Y.~W. Teh, D.~Newman, and M.~Welling}, {\em {A collapsed variational
  Bayesian inference algorithm for latent Dirichlet allocation}}, in Advances
  in neural information processing systems, 2007, pp.~1353--1360.

\bibitem{tyagi2014learning}
{\sc H.~Tyagi and V.~Cevher}, {\em {Learning non-parametric basis independent
  models from point queries via low-rank methods}}, Applied and Computational
  Harmonic Analysis, 37 (2014), pp.~389--412.

\bibitem{vershynin_2012}
{\sc R.~Vershynin}, {\em {Introduction to the non-asymptotic analysis of random
  matrices}}, in Compressed Sensing: Theory and Applications, Y.~C. Eldar and
  G.~Kutyniok, eds., Cambridge University Press, 2012, pp.~210--268.
  
\bibitem{zahm2018gradient}
{\sc O.~Zahm, P.~Constantine, C.~Prieur and Y.~Marzouk}, {\em {Gradient-based 
  dimension reduction of multivariate vector-valued functions}}, SIAM Journal on
  Scientific Computing, 42 (2020), pp.~A534--A558.

\end{thebibliography}

